Measuring Hadronic Higgs Boson Branching Ratios at Future Lepton Colliders

We present a novel strategy for the simultaneous measurement of Higgs-boson branching ratios into gluons and light quarks at a future lepton collider operating in the Higgs-factory mode. Our method is based on template fits to global event-shape observables, and in particular fractional energy correlations, thereby exploiting differences in the QCD radiation patterns of quarks and gluons. In a constrained fit of the deviations of the light-flavour hadronic Higgs-boson branching ratios from their Standard Model expectations, based on an integrated luminosity of $5\,\text{ab}^{-1}$, we obtain $68\%$ confidence level limits of $\mu_{gg}=1 \pm 0.05$ and $\mu_{q\bar{q}}<21$.

==> global.tex <==
%= math ===========================================
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{array}
\usepackage{calc}
\usepackage{longtable}
\usepackage{multirow,booktabs}
%= graphics =======================================
\usepackage{relsize}
%\usepackage{pstricks}
\usepackage{graphicx}
\usepackage{xspace}
\usepackage{units}
\usepackage{afterpage}
\usepackage{placeins}
%\usepackage{graphpap}
%= citations ======================================
\renewcommand{\theequation}{\arabic{section}.\arabic{equation}}
\numberwithin{equation}{section}
\usepackage{mciteplus}
%= layout =========================================
%\usepackage[a4paper,pdfborder={0 0 0}]{hyperref}

\RequirePackage{hyperref}
\hypersetup{pdfborder={0 0 0},unicode}

\usepackage[format=hang,labelfont=bf,hypcap=true]{caption}
\usepackage{subcaption}
\usepackage{sectsty}
\allsectionsfont{\sffamily}
\subsubsectionfont{\mdseries\itshape\large}
\setlength{\parindent}{0mm}
\setlength{\hoffset}{-1.75cm}
\setlength{\textwidth}{16.5truecm}
\setlength{\textheight}{24cm}
\setlength{\topmargin}{0mm}
\setlength{\headheight}{0mm}
\setlength{\headsep}{0mm}
\setlength{\parskip}{1mm}
\setlength{\mathindent}{2ex}
\makeatletter
\DeclareRobustCommand*{\bfseries}{%
  \not@math@alphabet\bfseries\mathbf
  \fontseries\bfdefault\selectfont
  \boldmath
}
\makeatother
\let\spreprint\empty
\newcommand{\preprint}[1]{\def\spreprint{\protect#1}}
\let\sinstitute\empty
\newcommand{\institute}[1]{\def\sinstitute{\protect#1}}
\makeatletter
\renewcommand{\maketitle}{\begingroup
  \null\thispagestyle{empty}%
    \ifx\spreprint\empty
      \vskip 5ex
    \else
      \flushright\large\spreprint\vskip 2ex
    \fi
    \vskip 5ex
    \flushleft
      {\sffamily\bfseries\huge\@title}\vskip 6ex
      \@author\vskip 2ex
      \ifx\sinstitute\empty
      \else
        {\small\sinstitute}
      \fi
    \vskip 5ex
  \endgroup
}
\makeatother
\renewenvironment{abstract}{\begin{center}
  {\large\sffamily\bfseries Abstract: }
  \begin{minipage}[t]{0.75\textwidth}
}{\end{minipage}\end{center}\vskip 10ex}
\newenvironment{stress}{\vskip 2ex
  \hspace*{2ex}\begin{minipage}{\textwidth-4ex}
  \em}{\end{minipage}\vskip 2ex}
\newcommand{\myfigure}[3]{
  \begin{figure}[#1]
    \begin{center}
      #2\\
      \parbox[t]{\widthof{#2}}{\caption{#3}}
    \end{center}
  \end{figure}
}
\newcommand{\mytable}[3]{
  \begin{table}[#1]
    \begin{center}
      #2\\
      \parbox[t]{\widthof{#2}}{\caption{#3}}
    \end{center}
  \end{table}
}
%= equation numeration scheme =====================
\renewcommand{\theequation}{\arabic{section}.\arabic{equation}}
\numberwithin{equation}{section}
%= abbreviations ==================================
\DeclareRobustCommand{\plusplus}{\raisebox{0.2ex}{\smaller++}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Physics macros
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{macros_physics}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Section references
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{macros_refs}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Experiments / Machines
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{macros_collabs}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Software names
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{macros_codes}




==> macros_codes.tex <==
%== ME+PS methods ======================================
%
%
\newcommand{\MCatNLO}{M\protect\scalebox{0.8}{C}@N\protect\scalebox{0.8}{LO}\xspace}
\newcommand{\POWHEG}{P\protect\scalebox{0.8}{OWHEG}\xspace}
\newcommand{\LOPS}{LO$\otimes$PS\xspace}
\newcommand{\MCatLO}{M\protect\scalebox{0.8}{C}@L\protect\scalebox{0.8}{O}\xspace}
\newcommand{\MEC}{M\scalebox{0.8}{E}C\xspace}
\newcommand{\MEPS}{M\scalebox{0.8}{E}P\scalebox{0.8}{S}\xspace}
\newcommand{\UMEPS}{UM\scalebox{0.8}{E}P\scalebox{0.8}{S}\xspace}
\newcommand{\NLOPS}{N\scalebox{0.8}{LO}P\scalebox{0.8}{S}\xspace}
\newcommand{\NNLOPS}{NN\scalebox{0.8}{LO}P\scalebox{0.8}{S}\xspace}
\newcommand{\UNLOPS}{UN\scalebox{0.8}{LO}P\scalebox{0.8}{S}\xspace}
\newcommand{\UNNLOPS}{UNN\scalebox{0.8}{LO}P\scalebox{0.8}{S}\xspace}
\newcommand{\MENLOPS}{ME\protect\scalebox{0.8}{NLO}PS\xspace}
\newcommand{\MEPSatLO}{M\protect\scalebox{0.8}{E}P\protect\scalebox{0.8}{S}@L\protect\scalebox{0.8}{O}\xspace}
\newcommand{\MEPSatNLO}{M\protect\scalebox{0.8}{E}P\protect\scalebox{0.8}{S}@N\protect\scalebox{0.8}{LO}\xspace}
\newcommand{\MINLO}{MIN\protect\scalebox{0.8}{LO}\xspace}
%
% == LO ME codes & methods ===============================
%
%
\newcommand{\Haag}{H\protect\scalebox{0.8}{AAG}\xspace}
\newcommand{\Sarge}{S\protect\scalebox{0.8}{ARGE}\xspace}
\newcommand{\Rambo}{R\protect\scalebox{0.8}{AMBO}\xspace}
\newcommand{\Vegas}{V\protect\scalebox{0.8}{EGAS}\xspace}
\newcommand{\Alpha}{A\protect\scalebox{0.8}{LPHA}\xspace}
\newcommand\ALPHA{\Alpha}
\newcommand{\Alpgen}{A\protect\scalebox{0.8}{LPGEN}\xspace}
\newcommand\alpgen{\Alpgen}
\newcommand{\Madgraph}{M\protect\scalebox{0.8}{AD}G\protect\scalebox{0.8}{RAPH}\xspace}
\newcommand\MADGRAPH{\Madgraph}
\newcommand{\Madevent}{M\protect\scalebox{0.8}{AD}E\protect\scalebox{0.8}{VENT}\xspace}
\newcommand{\Helac}{H\protect\scalebox{0.8}{ELAC}\xspace}
\newcommand{\Phegas}{P\protect\scalebox{0.8}{HEGAS}\xspace}
\newcommand{\Whizard}{W\protect\scalebox{0.8}{HIZARD}\xspace}
\newcommand{\OmegaCode}{O\protect\scalebox{0.8}{'MEGA}\xspace}
\newcommand{\Helas}{H\protect\scalebox{0.8}{ELAS}\xspace}
\newcommand\HELAS{\Helas}
\newcommand{\Calchep}{C\protect\scalebox{0.8}{ALC}H\scalebox{0.8}{EP}\xspace}
\newcommand{\Comphep}{C\protect\scalebox{0.8}{OMP}H\scalebox{0.8}{EP}\xspace}
%
% == event generators ======================================
%
%
\newcommand{\Herwig}{H\protect\scalebox{0.8}{ERWIG}\xspace}
\newcommand{\Jimmy}{J\protect\scalebox{0.8}{IMMY}\xspace}
\newcommand\herwig{\Herwig}
\newcommand\jimmy{\textsc{Jimmy}\xspace}
\newcommand\herwigjimmy{\Herwig/\jimmy}
\newcommand\herwigsix{\Herwig~6\xspace}
\newcommand\herwigpp{\Herwig\plusplus\xspace}
\newcommand{\HerwigPP}{\herwigpp}
\newcommand{\HERWIG}{\Herwig}
\newcommand{\Herwigpp}{H\protect\scalebox{0.8}{ERWIG++}\xspace}
\newcommand{\Ariadne}{A\protect\scalebox{0.8}{RIADNE}\xspace}
\newcommand\ariadne{\Ariadne}
\newcommand{\Pythia}{P\protect\scalebox{0.8}{YTHIA}\xspace}
\newcommand\pythia{\Pythia}
\newcommand\pythiasix{\Pythia~6\xspace}
\newcommand\pythiaseven{\Pythia~7\xspace}
\newcommand\pythiaeight{\Pythia~8\xspace}
\newcommand{\Jetset}{J\protect\scalebox{0.8}{ETSET}\xspace}
\newcommand\jetset{\Jetset}
\newcommand{\Vincia}{V\protect\scalebox{0.8}{INCIA}\xspace}
\newcommand{\VINCIA}{\Vincia}
\newcommand{\ThePEG}{T\protect\scalebox{0.8}{he}P\protect\scalebox{0.8}{EG}\xspace}
\newcommand{\Phojet}{P\protect\scalebox{0.8}{HOJET}\xspace}
\newcommand\phojet{\Phojet\xspace}
\newcommand{\Epos}{E\protect\scalebox{0.8}{POS}\xspace}
\newcommand\epos{\Epos\xspace}
\newcommand{\MLM}{M\protect\scalebox{0.8}{LM}\xspace}
%
% == NLO matching generators ======================================
%
%
\newcommand{\aMCatNLO}{aM\protect\scalebox{0.8}{C}@N\protect\scalebox{0.8}{LO}\xspace}
\newcommand{\PowhegBox}{P\protect\scalebox{0.8}{OWHEG}B\protect\scalebox{0.8}{OX}\xspace}
\newcommand{\POWHEGBOX}{\PowhegBox}
%
% == Resummation codes ==================================
%
%
\newcommand{\HRes}{HR\protect\scalebox{0.8}{ES}\xspace}
\newcommand{\HqT}{H\protect\scalebox{0.8}{qT}\xspace}
\newcommand{\Resbos}{R\protect\scalebox{0.8}{ES}B\protect\scalebox{0.8}{OS}\xspace}
\newcommand{\ResBos}{R\protect\scalebox{0.8}{ES}B\protect\scalebox{0.8}{OS}\xspace}
%
% == NLO ME tools and codes =============================
%
%
\newcommand{\HelacNLO}{H\protect\scalebox{0.8}{ELAC}-NLO\xspace}
\newcommand{\AutoTools}{A\protect\scalebox{0.8}{UTO}T\protect\scalebox{0.8}{OOLS}\xspace}
\newcommand{\CutTools}{C\protect\scalebox{0.8}{UT}T\protect\scalebox{0.8}{OOLS}\xspace}
\newcommand{\Gosam}{G\protect\scalebox{0.8}{O}S\protect\scalebox{0.8}{AM}\xspace}
\newcommand{\Samurai}{S\protect\scalebox{0.8}{AMURAI}\xspace}
\newcommand{\Collier}{C\protect\scalebox{0.8}{OLLIER}\xspace}
\newcommand{\Ninja}{N\protect\scalebox{0.8}{INJA}\xspace}
\newcommand{\BlackHat}{B\protect\scalebox{0.8}{LACK}H\protect\scalebox{0.8}{AT}\xspace}
\newcommand{\Blackhat}{B\protect\scalebox{0.8}{LACK}H\protect\scalebox{0.8}{AT}\xspace}
\newcommand{\MadLoop}{M\protect\scalebox{0.8}{AD}L\protect\scalebox{0.8}{OOP}\xspace}
\newcommand{\OpenLoops}{O\protect\scalebox{0.8}{PEN}L\protect\scalebox{0.8}{OOPS}\xspace}
\newcommand{\LoopTools}{L\protect\scalebox{0.8}{OOP}T\protect\scalebox{0.8}{OOLS}\xspace}
\newcommand{\FormCalc}{F\protect\scalebox{0.8}{ORM}C\protect\scalebox{0.8}{ALC}\xspace}
\newcommand{\QCDLoop}{QCDL\protect\scalebox{0.8}{OOP}\xspace}
\newcommand{\OneLoop}{O\protect\scalebox{0.8}{NE}L\protect\scalebox{0.8}{OOP}\xspace}
\newcommand{\MCFM}{M\protect\scalebox{0.8}{C}F\protect\scalebox{0.8}{M}\xspace}
\newcommand{\Njet}{N\protect\scalebox{0.8}{JET}\xspace}
\newcommand{\NLOJETpp}{N\protect\scalebox{0.8}{LOJET++}\xspace}
\newcommand{\Jetphox}{J\protect\scalebox{0.8}{ET}P\protect\scalebox{0.8}{HOX}\xspace}
\newcommand{\Diphox}{D\protect\scalebox{0.8}{I}P\protect\scalebox{0.8}{HOX}\xspace}
%
% == Subtraction tools =====================================
%
%
\newcommand{\MadDipole}{M\protect\scalebox{0.8}{AD}D\protect\scalebox{0.8}{IPOLE}\xspace}
\newcommand{\AutoDipole}{A\protect\scalebox{0.8}{UTO}D\protect\scalebox{0.8}{IPOLE}\xspace}
\newcommand{\MadFKS}{M\protect\scalebox{0.8}{AD}FKS\xspace}
\newcommand{\Matchbox}{M\protect\scalebox{0.8}{ATCH}B\protect\scalebox{0.8}{OX}\xspace}
%
% == Sherpa stuff ====================================
%
%
\newcommand{\Sherpa}{S\protect\scalebox{0.8}{HERPA}\xspace}
\newcommand{\SHERPA}{\Sherpa}
\newcommand{\Comix}{C\protect\scalebox{0.8}{OMIX}\xspace}
\newcommand{\Apacic}{A\protect\scalebox{0.8}{PACIC\plusplus}\xspace}
\newcommand{\Amegic}{A\protect\scalebox{0.8}{MEGIC\plusplus}\xspace}
\newcommand{\CSShower}{CSS\protect\scalebox{0.8}{hower}\xspace}
\newcommand{\CSS}{C\protect\scalebox{0.8}{SS}\xspace}
\newcommand{\Dire}{D\protect\scalebox{0.8}{IRE}\xspace}
\newcommand{\Ahadic}{A\protect\scalebox{0.8}{HADIC\plusplus}\xspace}
\newcommand{\Adicic}{A\protect\scalebox{0.8}{DICIC\plusplus}\xspace}
\newcommand{\Hadrons}{H\protect\scalebox{0.8}{ADRONS\plusplus}\xspace}
\newcommand{\Photons}{P\protect\scalebox{0.8}{HOTONS\plusplus}\xspace}
\newcommand\sherpa{\Sherpa}
%
% == event generator tuning & validation ===================
%
%
\newcommand\thepeg{\ThePEG}
\newcommand{\HEJ}{H\protect\scalebox{0.8}{EJ}\xspace}
\newcommand{\Professor}{P\protect\scalebox{0.8}{ROFESSOR}\xspace}
\newcommand\professor{\Professor}
\newcommand{\xfig}{XF\protect\scalebox{0.8}{IG}}
\newcommand{\matplotlib}{M\protect\scalebox{0.8}{AT}P\protect\scalebox{0.8}{LOT}L\protect\scalebox{0.8}{IB}\xspace}
\newcommand{\Rivet}{R\protect\scalebox{0.8}{IVET}\xspace}
\newcommand\rivet{\Rivet}
\newcommand{\Agile}{A\protect\scalebox{0.8}{GILE}\xspace}
\newcommand\agile{\Agile}
\newcommand{\HepData}{H\protect\scalebox{0.8}{EP}D\protect\scalebox{0.8}{ATA}\xspace}
\newcommand\hepdata{\HepData}
\newcommand{\HepMC}{H\protect\scalebox{0.8}{EP}MC\xspace}
\newcommand\hepmc{\HepMC}
\newcommand{\HZTool}{HZT\protect\scalebox{0.8}{OOL}\xspace}
\newcommand\hztool{\HZTool}
%
% == other codes ==================================
%
%
\newcommand{\FeynRules}{F\protect\scalebox{0.8}{EYN}R\protect\scalebox{0.8}{ULES}\xspace}
\newcommand{\SpringBases}{S\protect\scalebox{0.8}{PRING/}B\protect\scalebox{0.8}{ASES}\xspace}

\newcommand{\Charybdis}{C\protect\scalebox{0.8}{HARYBDIS}\xspace}
\newcommand{\Fastjet}{F\protect\scalebox{0.8}{AST}J\protect\scalebox{0.8}{ET}\xspace}
\newcommand{\EvtGen}{E\protect\scalebox{0.8}{VT}G\protect\scalebox{0.8}{EN}\xspace}
\newcommand{\TAUOLA}{T\protect\scalebox{0.8}{AUOLA}\xspace}
\newcommand{\Photos}{P\protect\scalebox{0.8}{HOTOS}\xspace}
\newcommand{\Jade}{J\protect\scalebox{0.8}{ADE}\xspace}
\newcommand{\Durham}{D\protect\scalebox{0.8}{URHAM}\xspace}
\newcommand\charybdis{\Charybdis}
\newcommand\fastjet{\FastJet}
\newcommand\evtgen{\EvtGen}
\newcommand\Tauola{\TAUOLA}
\newcommand\tauola{\TAUOLA}
\newcommand\photos{\PHOTOS}
\newcommand\FEWZ{F\protect\scalebox{0.8}{EWZ}\xspace}
\newcommand\jade{\Jade}
\newcommand\durham{\Durham}
\newcommand\FONLL{F\protect\scalebox{0.8}{ONLL}\xspace}
\newcommand\FONLLA{F\protect\scalebox{0.8}{ONLL}-A\xspace}
\newcommand\FONLLB{F\protect\scalebox{0.8}{ONLL}-B\xspace}
\newcommand\FONLLC{F\protect\scalebox{0.8}{ONLL}-C\xspace}

%
% == PDF stuff ================================== 
%
%
\newcommand{\LHAPDF}{L\protect\scalebox{0.8}{HA}PDF\xspace}
\newcommand{\lhapdf}{\LHAPDF}
\newcommand{\lostar}{\ensuremath{\text{LO}*}\xspace}
\newcommand{\cteq}[1]{\ensuremath{\text{CTEQ#1}}\xspace}




==> macros_collabs.tex <==
\newcommand{\Contur}{C\protect\scalebox{0.8}{ONTUR}\xspace}
\newcommand{\Apprentice}{A\protect\scalebox{0.8}{PPRENTICE}\xspace}
\newcommand{\Caesar}{C\protect\scalebox{0.8}{AESAR}\xspace}
\newcommand{\ARES}{A\protect\scalebox{0.8}{RES}\xspace}

\newcommand\fnal{F\scalebox{0.8}{NAL}\xspace}

\newcommand\tevatron{T\protect\scalebox{0.8}{EVATRON}\xspace}
\newcommand\Tevatron{\protect\tevatron}
\newcommand\runi{Run-\textsmaller{I}\xspace}
\newcommand\runii{Run-\textsmaller{II}\xspace}
\newcommand\runiia{Run-\textsmaller{II}a\xspace}
\newcommand\runiib{Run-\textsmaller{II}b\xspace}
\newcommand\cdf{CDF\xspace}
\newcommand\CDF{\cdf}
\newcommand\dzero{D\O\xspace}
\newcommand{\DO}{\dzero}

\newcommand\cern{C\scalebox{0.8}{ERN}\xspace}

\newcommand\babar{B\scalebox{0.8}{ABAR}\xspace}
\newcommand\lep{L\scalebox{0.8}{EP}\xspace}
\newcommand\lepi{L\scalebox{0.8}{EP}~1\xspace}
\newcommand\LEP{\lep}
\newcommand\LEPI{\lepi}
\newcommand{\LEPOne}{L\protect\scalebox{0.8}{EP}1\xspace}
\newcommand\PETRA{P\scalebox{0.8}{ETRA}\xspace}
\newcommand\TOPAZ{T\scalebox{0.8}{OPAZ}\xspace}
\newcommand\AMY{A\scalebox{0.8}{MY}\xspace}
\newcommand\CELLO{C\scalebox{0.8}{ELLO}\xspace}
\newcommand\TASSO{T\scalebox{0.8}{ASSO}\xspace}
\newcommand\HERA{H\scalebox{0.8}{ERA}\xspace}
\newcommand\lepii{L\scalebox{0.8}{EP}~2\xspace}
\newcommand\ALEPH{A\scalebox{0.8}{LEPH}\xspace}
\newcommand{\Aleph}{A\protect\scalebox{0.8}{LEPH}\xspace}
\newcommand\delphi{D\scalebox{0.8}{ELPHI}\xspace}
\newcommand\DELPHI{\delphi}
\newcommand\OPAL{\opal}
\newcommand\opal{O\scalebox{0.8}{PAL}\xspace}
\newcommand{\Opal}{O\protect\scalebox{0.8}{PAL}\xspace}
\newcommand\Delphi{\delphi}
\newcommand\lthree{L3\xspace}
\newcommand\lhc{L\protect\scalebox{0.8}{HC}\xspace}
\newcommand\LHC{L\protect\scalebox{0.8}{HC}\xspace}
\newcommand\ATLAS{\atlas}
\newcommand\atlas{A\protect\scalebox{0.8}{TLAS}\xspace}
\newcommand\CMS{\cms}
\newcommand\cms{C\protect\scalebox{0.8}{MS}\xspace}
\newcommand\TOTEM{\totem}
\newcommand\totem{T\protect\scalebox{0.8}{OTEM}\xspace}
\newcommand\ALICE{\alice}
\newcommand\alice{A\protect\scalebox{0.8}{LICE}\xspace}
\newcommand\LHCb{\lhcb}
\newcommand\lhcb{L\scalebox{0.8}{HC}B\xspace}

\newcommand\rhic{R\scalebox{0.8}{HIC}\xspace}
\newcommand\SLD{S\scalebox{0.8}{LD}\xspace}
\newcommand\SLC{S\scalebox{0.8}{LC}\xspace}

\newcommand\JADE{J\scalebox{0.8}{ADE}\xspace}
\newcommand\hera{H\scalebox{0.8}{ERA}\xspace}
\newcommand\hone{H1\xspace}
\newcommand\HONE{\hone}
\newcommand\zeus{Z\scalebox{0.8}{EUS}\xspace}
\newcommand\ZEUS{\zeus}

\newcommand\WMAP{W\scalebox{0.8}{MAP}\xspace}
\newcommand\PLANCK{P\scalebox{0.8}{LANCK}\xspace}
\newcommand\sld{SLD\xspace}

\newcommand\mcnet{MCnet\xspace}
\newcommand\pdg{PDG\xspace}
\newcommand\PDG{PDG\xspace}
\newcommand\spires{SPIRES\xspace}



==> macros_physics.tex <==
%%%% units
\newcommand{\Ummeter}{\ensuremath{\mathrm{mm}}\xspace}
\newcommand{\Umeter}{\ensuremath{\mathrm{m}}\xspace}
\newcommand{\Ufermi}{\ensuremath{\mathrm{fm}}\xspace}
\newcommand{\Umb}{\ensuremath{\mathrm{mb}}\xspace}
\newcommand{\UMeV}{\ensuremath{\mathrm{MeV}}\xspace}
\newcommand{\UGeV}{\ensuremath{\mathrm{GeV}}\xspace}
\newcommand{\UTeV}{\ensuremath{\mathrm{TeV}}\xspace}
\newcommand{\GeV}{\ensuremath{\mathrm{GeV}}\xspace}

% Kinematical quantities
\newcommand{\Ecm}{\ensuremath{E_{\mathrm{c.m.}}}\xspace}
\newcommand{\hatEcm}{\ensuremath{\hat{E}_{\mathrm{c.m.}}}\xspace}
\newcommand{\kt}{\ensuremath{k_\perp}\xspace}
\newcommand{\kT}{\kt}
\newcommand{\kperp}{\kt}
\newcommand{\sqrts}{\ensuremath{\sqrt{s}}\xspace}
\newcommand{\shat}{\ensuremath{\hat{s}}\xspace}
\newcommand{\mt}{\ensuremath{m_\perp}\xspace}
\newcommand{\pt}{\ensuremath{p_\perp}\xspace}
\newcommand{\ptzero}{\ensuremath{p_{\perp,0}}\xspace}
\newcommand{\ptmin}{\ensuremath{p_{\perp,\mathrm{min}}}\xspace}
\newcommand{\mT}{\mt}
\newcommand{\pT}{\pt}
\newcommand{\QT}{\ensuremath{Q_T}}
\newcommand{\pperp}{\pt}
% variants of pT that can take an argument
\newcommand{\mPerp}[1]{\ensuremath{m_{\perp #1}}\xspace}
\newcommand{\pPerp}[1]{\ensuremath{p_{\perp #1}}\xspace}

%%%% Reactions
\newcommand{\pp}{\ensuremath{pp}\xspace}
\newcommand{\ppbar}{\ensuremath{p\bar{p}}\xspace}
\newcommand{\epluseminus}{\ensuremath{e^+ e^-}\xspace}
\newcommand{\ee}{\epluseminus\xspace}
\newcommand{\ep}{\ensuremath{e^\pm p}\xspace}

%%%% Particles and their properties
\newcommand{\MW}{\ensuremath{m_W}}
\newcommand{\MH}{\ensuremath{m_H}}
\newcommand{\MZ}{\ensuremath{m_Z}}
\newcommand{\MT}{\ensuremath{m_t}}
\newcommand{\MB}{\ensuremath{m_b}}
\newcommand{\MC}{\ensuremath{m_c}}
\newcommand{\MS}{\ensuremath{m_s}}
\newcommand{\MD}{\ensuremath{m_d}}
\newcommand{\MU}{\ensuremath{m_u}}
\newcommand{\Mtau}{\ensuremath{m_\tau}}
\newcommand{\GW}{\ensuremath{\Gamma_W}}
\newcommand{\GZ}{\ensuremath{\Gamma_Z}}
\newcommand{\GT}{\ensuremath{\Gamma_t}}

%%%% Couplings
\newcommand{\MSbar}{\ensuremath{\overline{\mathrm{MS}}}}
\newcommand{\llalphaps}{\ensuremath{\alpha_{\text{s,PS}}}\xspace}
\newcommand{\alphaS}{\ensuremath{\alpha_\text{s}}\xspace}
\newcommand{\alphaSn}[1]{\ensuremath{\alpha^#1_\text{s}}\xspace}
\newcommand{\alphaW}{\ensuremath{\alpha_\text{w}}\xspace}
\newcommand{\Nc}{\ensuremath{N_c}}
\newcommand{\nf}{\ensuremath{n_f}}
\newcommand{\CF}{\ensuremath{C_F}}
\newcommand{\CA}{\ensuremath{C_A}}
\newcommand{\TR}{\ensuremath{T_R}}
\newcommand{\LambdaQCD}{\ensuremath{\Lambda_\text{QCD}}\xspace}
\newcommand{\gs}{\ensuremath{g_s}}
\newcommand{\gW}{\ensuremath{g_W}}
\newcommand{\gFermi}{\ensuremath{G_F}}
\newcommand{\GF}{\gFermi}
\newcommand{\sinW}{\ensuremath{\sin\theta_W}}
\newcommand{\cosW}{\ensuremath{\cos\theta_W}}
\newcommand{\sinSqW}{\ensuremath{\sin^2\theta_W}}
\newcommand{\cosSqW}{\ensuremath{\cos^2\theta_W}}
\newcommand{\BR}[1]{\ensuremath{\mathcal{BR}_{#1}}}
\newcommand{\DeltaPom}{\ensuremath{{\Delta_{\mathbf{P}}}}}

\newcommand{\pdf}[2]{\ensuremath{f_{#2/#1}}}
\newcommand{\ff}[2]{\ensuremath{D_{#2/#1}}}
\newcommand{\muR}{\ensuremath{\mu_R}}
\newcommand{\muF}{\ensuremath{\mu_F}}
\newcommand{\muQ}{\ensuremath{\mu_Q}}
\newcommand{\Ecms}{\ensuremath{E_\mathrm{cms}}}
\newcommand{\mucut}{\ensuremath{\mu_{Q_\mathrm{cut}}}}
\newcommand{\ycut}{\ensuremath{y_\mathrm{cut}}}
\newcommand{\Qcut}{\ensuremath{Q_\mathrm{cut}}}
\newcommand{\QcutSq}{\ensuremath{Q_\mathrm{cut}^2}}
\newcommand{\Qiso}{\ensuremath{Q_\mathrm{iso}}}
\newcommand{\tcut}{\ensuremath{t_\mathrm{c}}}
\newcommand{\nmax}{\ensuremath{N_\mathrm{max}}}
\newcommand{\nmin}{\ensuremath{N_\mathrm{min}}}
\newcommand{\tnmax}{\ensuremath{t_\nmax}}
\newcommand{\tcutQED}{\ensuremath{t_{\mathrm{c},\mathrm{(QED)}}}}
\newcommand{\alphacut}{\ensuremath{\alpha_{\mathrm{cut}}}}

%%%% Bits of calculations
\newcommand{\tFFDipole}[3]{\ensuremath{{\tilde{\mathcal{D}}_{#1#2;#3}}}}
\newcommand{\Dipole}{\ensuremath{{\mathcal{D}}}}
\newcommand{\tDipole}{\ensuremath{\tilde{\mathcal{D}}}}
\newcommand{\IntDip}{\ensuremath{{\mathcal{I}^{(\mathcal{D})}}}}
\newcommand{\IntDipole}[2]{\ensuremath{{\mathcal{I}^{(\mathcal{D})}_{#1;#2}}}}
\newcommand{\FFDipole}[3]{\ensuremath{{\mathcal{D}_{#1#2;#3}}}}
\newcommand{\FIDipole}[3]{\ensuremath{{\mathcal{D}_{#1#2}^{#3}}}}
\newcommand{\IFDipole}[3]{\ensuremath{{\mathcal{D}^{#1#2}_{#3}}}}
\newcommand{\IIDipole}[3]{\ensuremath{{\mathcal{D}^{#1#2;#3}}}}
\newcommand{\DipOp}[1]{\ensuremath{{\mathbf{D}}(#1)}}
\newcommand{\IntDipOp}[2]{\ensuremath{{\mathbf{I}}(#1;\,#2)}}
\newcommand{\IntDipOpFF}[2]{\ensuremath{{\mathbf{I}}_{FF}(#1;\,#2)}}
\newcommand{\IntDipOpFI}[2]{\ensuremath{{\mathbf{I}}_{FI}(#1;\,#2)}}
\newcommand{\IntDipOpIF}[2]{\ensuremath{{\mathbf{I}}_{IF}(#1;\,#2)}}
\newcommand{\IntDipOpII}[2]{\ensuremath{{\mathbf{I}}_{II}(#1;\,#2)}}
\newcommand{\Eikonal}[4]{\ensuremath{{\mathcal{W}(#1,\,#2;\,#3,\,#4)}}}
\newcommand{\Eik}{\ensuremath{{\mathrm{W}}}}
\newcommand{\Ampl}{\ensuremath{{\mathcal{A}}}}
\newcommand{\Prob}{\ensuremath{{\mathcal{P}}}}
\newcommand{\Sub}{\ensuremath{{\mathcal{S}}}}
\newcommand{\SubKernel}{\ensuremath{\tilde{\mathcal S}}}
\newcommand{\SubKInt}{\ensuremath{\tilde{S}}}
\newcommand{\Born}{\ensuremath{{\mathcal{B}}}}
\newcommand{\Hard}{\ensuremath{{\mathcal{H}}}}
\newcommand{\Evol}[2]{\ensuremath{{\mathcal{E}_{#1}^{(#2)}}}}
\newcommand{\EvolIn}[3]{\ensuremath{{\mathcal{E}_{#1}^{(#2,<#3)}}}}
\newcommand{\bBorn}{\ensuremath{\bar{\mathcal{B}}}}
\newcommand{\tBorn}{\ensuremath{\tilde{\mathcal{B}}}}
\newcommand{\Real}{\ensuremath{{\mathcal{R}}}}
\newcommand{\Subtraction}{\ensuremath{{\mathcal{S}}}}
\newcommand{\IntSubtraction}{\ensuremath{\mathcal{I}^{(\mathcal{S})}}}
\newcommand{\RealS}{\ensuremath{{\mathcal{R}}^{(\mathrm{S})}}}
\newcommand{\RealH}{\ensuremath{{\mathcal{R}}^{(\mathrm{H})}}}
\newcommand{\Virtual}{\ensuremath{{\mathcal{V}}}}
\newcommand{\Kernel}{\ensuremath{\mathcal{K}}}
\newcommand{\KernelIn}[1]{\ensuremath{\mathcal{K}^{<#1}}}
\newcommand{\BornPS}{\ensuremath{\Phi_{{\mathcal{B}}}}}
\newcommand{\RealPS}{\ensuremath{\Phi_{{\mathcal{R}}}}}
\newcommand{\OnePS}{\ensuremath{\Phi_{1}}}
\newcommand{\PS}[1]{\ensuremath{\Phi_{#1}}}
\newcommand{\LO}{\ensuremath{\mathrm{LO}}}
\newcommand{\NLO}{\ensuremath{\mathrm{NLO}}}
\newcommand{\NNLO}{\ensuremath{\mathrm{NNLO}}}
\newcommand{\Me}{\ensuremath{\mathcal{M}}}
\newcommand{\ME}[1]{\ensuremath{\mathcal{M}^{({#1})}}}
\newcommand{\MEstar}[1]{\ensuremath{\mathcal{M}^{*({#1})}}}
\newcommand{\Splitting}{\ensuremath{\mathcal{P}}}
\newcommand{\splitting}[2]{\ensuremath{\mathcal{P}_{#1#2}}}
\newcommand{\Nsplitting}[2]{\ensuremath{\hat{\mathcal{P}}_{#1#2}}}
\newcommand{\helsum}{\ensuremath{\bar\Sigma_{\mathrm hel.}}}
\newcommand{\prefD}{\ensuremath{\mu^{4-D}}}
\newcommand{\LoopD}[1]{\ensuremath{\frac{\dD{#1}}{(2\pi)^D}}}
\newcommand{\Tr}[1]{\ensuremath{\mathrm{Tr}\left[#1\right]}}
\newcommand{\sla}[1]{\ensuremath{{#1\kern-0.45em/}}}

\newcommand{\bV}{{\bf V}}

\newcommand{\lagrange}{\ensuremath{\mathcal{L}}}
\newcommand{\lumi}{\ensuremath{\mathcal{L}}}
\newcommand{\sigtot}{\ensuremath{\sigma_{\mathrm{tot}}}}
\newcommand{\sigeff}{\ensuremath{\sigma_{\mathrm{eff}}}}
\newcommand{\sigel}{\ensuremath{\sigma_{\mathrm{el}}}}
\newcommand{\siginel}{\ensuremath{\sigma_{\mathrm{inel}}}}
\newcommand{\BRatio}[1]{\ensuremath{\mathrm{BR}_{#1}}}
\newcommand{\Rate}[1]{\ensuremath{\mathfrak{R}_{#1}}}

\newcommand{\aCDR}{\ensuremath{a^{\mathrm{CDR}}}}

\newcommand{\antikT}[1]{anti-$k_T$~($D=0.#1$)}
\newcommand{\midpoint}{M\protect\scalebox{0.8}{ID}P\protect\scalebox{0.8}{OINT}\xspace}

\newcommand{\chisq}{\ensuremath{\chi^2}\xspace}


==> macros_refs.tex <==
\newcommand{\EqRef}[1]{Eq.~\eqref{#1}\xspace}
\newcommand{\EqsRef}[2]{Eqs.~\eqref{#1} -- \eqref{#2}\xspace}
\newcommand{\EqRefs}[2]{Eqs.~\eqref{#1} and \eqref{#2}\xspace}
\newcommand{\EqRefsT}[3]{Eqs.~\eqref{#1}, \eqref{#2} and \eqref{#3}\xspace}
\newcommand{\PageRef}[1]{page~\pageref{#1}\xspace}
\newcommand{\PagesRef}[2]{pages~\pageref{#1} -- \pageref{#2}\xspace}
\newcommand{\ChapRef}[1]{Chapter~\ref{#1}\xspace}
\newcommand{\ChapRefs}[2]{Chapters~\ref{#1} and \ref{#2}\xspace}
\newcommand{\ChapsRef}[2]{Chapters~\ref{#1} -- \ref{#2}\xspace}
\newcommand{\SecRef}[1]{Section~\ref{#1}\xspace}
\newcommand{\SecRefs}[2]{Sections~\ref{#1} and \ref{#2}\xspace}
\newcommand{\SecsRef}[2]{Sections~\ref{#1} -- \ref{#2}\xspace}
\newcommand{\AppRef}[1]{Appendix~\ref{#1}\xspace}
\newcommand{\AppRefs}[2]{Appendics~\ref{#1} and \ref{#2}\xspace}
\newcommand{\FigRef}[1]{Fig.~\ref{#1}\xspace}
\newcommand{\FigRefs}[2]{Figs.~\ref{#1} and~\ref{#2}\xspace}
\newcommand{\FigsRef}[2]{Figs.~\ref{#1} -- \ref{#2}\xspace}
\newcommand{\TabRef}[1]{Tab.~\ref{#1}\xspace}
\newcommand{\TabsRef}[1]{Tabs.~\ref{#1}\xspace}
\newcommand{\mycaption}[3]{\parbox{.8\textwidth}{\caption[#1]{#2\label{#3}}}}
\newcommand{\mycaptionwide}[3]{\parbox{\textwidth}{\caption[#1]{#2\label{#3}}}}
\newcommand{\mycaptionhalf}[3]{\parbox{.4\textwidth}{\caption[#1]{#2\label{#3}}}}
\newcommand{\eg}{{\it e.g.}\xspace}
\newcommand{\ie}{{\it i.e.}\xspace}
\newcommand{\cf}{{\it cf.}\xspace}
\newcommand{\gloss}[2]{{\bf #1:} #2}

